Unified Single-Image and Video Super-Resolution via Denoising Algorithms

Single Image Super-Resolution (SISR) aims to recover a high-resolution image from a given low-resolution version of it. Video Super Resolution (VSR) targets series of given images, aiming to fuse them to create a higher resolution outcome. Although SISR and VSR seem to have a lot in common, most SISR algorithms do not have a simple and direct extension to VSR. VSR is considered a more challenging inverse problem, mainly due to its reliance on a sub-pixel accurate motion-estimation, which has no parallel in SISR. Another complication is the dynamics of the video, often addressed by simply generating a single frame instead of a complete output sequence. In this work we suggest a simple and robust super-resolution framework that can be applied to single images and easily extended to video. Our work relies on the observation that denoising of images and videos is well-managed and very effectively treated by a variety of methods. We exploit the Plug-and-Play-Prior framework and the Regularization-by-Denoising (RED) approach that extends it, and show how to use such denoisers in order to handle the SISR and the VSR problems using a unified formulation and framework. This way, we benefit from the effectiveness and efficiency of existing image/video denoising algorithms, while solving much more challenging problems. More specifically, harnessing the VBM3D video denoiser, we obtain a strongly competitive motion-estimation free VSR algorithm, showing tendency to a high-quality output and fast processing.

==> main/05_convergence.tex <==
\section{Convergence}\label{SS:Convergence}
It is shown in \cite{ADMM_REF} that if the two terms being minimized in Equation (\ref{MAP_cost_split}), that is, the ML estimator and the prior, are closed proper and convex, and the unaugmented Lagrangian has a saddle point, then the ADMM is guaranteed to converge.
Optimality conditions are primal and dual feasibility. Primal feasibility is reached when $x=v$. Increasing $\rho$ will increase the penalty for $\|\x - \v\|_2^2$ and hence will guaranty primal feasibility. On the other hand, \cite{ADMM_REF} stresses that for dual feasibility, $\rho \left(\v_{k+1}-\v_{k}\right) \rightarrow 0$ must hold. Hence, although $\rho$ should be increased, this should be done with care, in order not to increase $\rho \left(\v_{k+1}-\v_{k}\right)$. $\rho$'s update in Algorithms \ref{ppp_algorithm} and \ref{red_algorithm} is meant to increase $\rho$ as long as $\rho \left(\v_{k+1}-\v_{k}\right)$ keeps decreasing.
PPP's convergence was proven and discussed in \cite{PPP_REF,PPP_CONVERGENCE_REF}, yet, since the Prior is unknown in this scheme, convergence is unclear.
RED, on the other hand, is shown to converge under mild conditions. (See \cite{RED_REF} for more details).
Indeed our experimental results show this as well.

Figure \ref{salesman_convergence} displays the PSNR during the iterations of RED-2 and PPP. The sharp drop in PSNR occurs when $\rho$ is decreased to ensure dual feasibility.
One can see that PPP converges slower, and is highly dependent on the $\rho$ update (the iteration is stuck till $\rho$ is decreased). RED-2, on the other hand, converges faster, and could have stopped the iteration earlier with almost the same PSNR score.
\begin{figure}[!htbp]
\includegraphics[scale=0.5]{./graphics/salesman_convergence.jpg}
\caption{PSNR during iteration of PPP and RED-2 on the \textsf{Salesman} sequence}
\label{salesman_convergence}
\end{figure}  

